Adaptive and Robust Watermark for Generative Tabular Data

In recent years, watermarking generative tabular data has become a prominent framework to protect against the misuse of synthetic data. However, while most prior work in watermarking methods for tabular data demonstrate a wide variety of desirable properties (e.g., high fidelity, detectability, robustness), the findings often emphasize empirical guarantees against common oblivious and adversarial attacks. In this paper, we study a flexible and robust watermarking algorithm for generative tabular data. Specifically, we demonstrate theoretical guarantees on the performance of the algorithm on metrics like fidelity, detectability, robustness, and hardness of decoding. The proof techniques introduced in this work may be of independent interest and may find applicability in other areas of machine learning. Finally, we validate our theoretical findings on synthetic and real-world tabular datasets.

==> experiment-old.tex <==
\section{Experiments}
\label{sec:experiment}
%
In this section, we empirically evaluate the our watermarking algorithm on a set of synthetic and real-world datasets to verify our theoretical claims. Formally, we seek to answer the following questions: (1) can our watermarking method ensure high data fidelity and downstream utility? (\Cref{sec:fidelity}); (2) is our watermarking method detectable for datasets of various size and distribution? (\Cref{sec:dectection}); (3) is our watermarking method robust against common adversarial attacks? (\Cref{sec:robustness}). 


\paragraph{Experimental Detail}
For all synthetic data experiments, we generate a dataset of size $2000 \times2$ using the standard Gaussian distribution for classification task. In this synthetic dataset, one column is chosen to be the $key$ column, and the other chosen as the $value$ column. For experiments on real-world datasets, we evaluate our technique on four real-world datasets of various sizes and distributions: Boston Housing and California Housing Price for regression task, as well as Adult and Wilt~\citep{misc_wilt_285} for classification task. For each dataset, we generate corresponding synthetic datasets using Gaussian Copula~\citep{masarotto2012gaussian}. We use Random Forest as the downstream machine learning algorithm for all datasets. For detection, the $z$-score threshold for the watermark to be detected is set to $1.96$, which corresponds to a false positive rate of $p=0.05$. 



%
\subsection{Synthetic Tabular Data}
First, we evaluate our algorithm on synthetic data to validate the our theoretical guarantees and performance sensitivity to selected parameters.


\paragraph{Fidelity} First, we verify that the watermark embedding procedure in \Cref{alg:fractional} maintains high data fidelity. In Figures \ref{fig:gaussian-hist} and \ref{fig:gaussian-hist-wm}, we show the two KDE plots showing a minimal difference between the data distribution before and after watermarking.

% In the second experiment, we generate multiple datasets, each containing 50 columns and varying numbers of rows from 20 to 100, to validate the effect that the row count has on the maximum achievable $z$-score. We repeat this process 5 times and take the average $z$-score. In Figure \ref{fig:z-score}, we find that as the number of rows in the dataset increases, so does the maximum possible $z$-score. This means that given a choice of $z$-score threshold, i) there is an increasing minimum number of total rows that the dataset must contain to achieve that score, and ii) as the number of rows increases, so does the number of rows that an attacker must sufficiently alter to break the watermark.

We further examine the effect on downstream utility with regard to different choices of the bin size $b$ in \Cref{alg:fractional}. For this experiment, we measure the downstream utility as the mean squared error for a classification task. Particularly, we vary the bin size $b$ between $10^{-4}$ and $10^{-1}$ (corresponding to between 10000 bins and 10 bins, respectively). We found that smaller bin size correspond to smaller MSE and higher downstream utility (\Cref{fig:gaussian-fidelity}). This behavior is as expected, since smaller bin size means the nearest green interval used for watermark embedding step in line 9 of \Cref{alg:fractional} is closer to the original data sample. 

\paragraph{Detectability} In addition to fidelity, we measure the detectability of our watermarking scheme by measuring the $z$-score on the watermarked dataset. 
On the other hand, we observe in \Cref{fig:gaussian-noise} that smaller bin size leads to lower $z$-score (higher $p$-value). That is, our watermarking scheme is more susceptible to additive noise attack    

\paragraph{Robustness} Finally, we consider the \textit{fidelity vs. robustness} trade-off that the \textit{bin size} parameter poses. We generate a dataset of size $2000\times2$ using the standard Gaussian distribution. The first column is chosen as the $key$ column and the other column is $value$, and we vary the \textit{bin size} between $10^{-4}$ and $10^{-1}$. The average mean squared error across 5 runs between the original data and the watermarked data for each \textit{bin size} is shown in Figure \ref{fig:gaussian-fidelity}. As expected, greater fidelity is maintained with smaller bins since adjusting the data to fall into the nearest green bin requires smaller perturbations. Figure \ref{fig:gaussian-noise} displays the accompanying susceptibility to noise that comes with smaller bins. Across 5 runs, we add zero-mean Gaussian noise with standard deviation varying from $10^{-3}$ to $10^{-1}$ to the watermarked data and measure the effect on the $z$-score. In each case, we find that smaller bins result in lower scores.

\paragraph{Classification}
To validate the effectiveness of our feature importance based pairing scheme, we generate a multi-class classification dataset of size $75\times75$ using scikit-learn, setting the number of classes to 5 and the number of informative features to 37. We create a set of column pairs using two different schemes: i) \emph{uniform}: features are paired uniformly at random and ii) \emph{feature importance}: sampling columns by treating their feature importance according to a Random Forest classifier as probabilities, pairing columns that are sampled one after the other. Using these two pairing schemes we create two watermarked datasets by watermarking 12 of the 37 available pairs, respectively.

For each of the watermarked datasets, we train a Random Forest classifier and use the resulting feature importance to drop subsets of columns varying in size from $20\%$ to $80\%$. The metric of interest in this experiment is the percentage of pairs retained after column dropping. Both columns in a pair must still remain in the dataset to be counted as a preserved pair. This entire process is repeated 5 times, and the averaged results are shown in Figure \ref{fig:classification-pairing}. The results show a significant increase in preserved pairs when the pairs are created using the feature importance scheme.

%
\begin{figure*}[ht]
    \centering
    \begin{subfigure}[b]{0.32\linewidth}
            \centering
            \includegraphics[height=3.85cm]{figures/histogram_original.png}
            \caption{KDE before watermark}
            \label{fig:gaussian-hist}
    \end{subfigure}
    \hfill 
    \begin{subfigure}[b]{0.32\linewidth}
            \centering
            \includegraphics[height=3.85cm]{figures/histogram_wm.png}
            \caption{KDE after watermark}
            \label{fig:gaussian-hist-wm}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\linewidth}
            \centering
            \includegraphics[height=3.85cm]{figures/zscore_vs_numrows.png}
            \caption{$z$-score with number of samples}
            \label{fig:z-score}
    \end{subfigure}
    \vfill
    \begin{subfigure}[b]{0.32\linewidth}
            \centering
            \includegraphics[height=3.85cm]
            {figures/fidelity.png}
            \caption{Fidelity with different bin sizes}
            \label{fig:gaussian-fidelity}
    \end{subfigure}
    \hfill 
    \begin{subfigure}[b]{0.32\linewidth}
            \centering
            \includegraphics[height=3.85cm]{figures/gaussian_noise.png}
            \caption{$z$-score with Gaussian noise}
            \label{fig:gaussian-noise}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\linewidth}
            \centering
            \includegraphics[height=3.85cm]{figures/preserved_vs_colsdropped.png}
            \caption{Robustness under PAIR}
            \label{fig:classification-pairing}
    \end{subfigure}
    \caption{
    (a) KDE plot of the Gaussian data before watermarking. (b) KDE plot of the Gaussian data after watermarking. (c) The maximum possible $z$-score increases with the number of rows in the dataset. (d) Smaller bin sizes result in higher fidelity (lower MSE) between the original data and the watermarked data. (e) Smaller bin sizes are more susceptible to noise, resulting in lower $z$-scores. Sigma corresponds to the standard deviation of the applied zero-mean Gaussian noise. (f) Pairing columns according to feature importance increases the pair preservation rate when the least important features are dropped. `Random' indicates random column pairings while `FI' indicates column pairings biased toward similar feature importances.}
    \label{fig:synthetic-data}
\end{figure*}
%
\subsection{Generative Tabular Data}
%
In addition to synthetic data, we evaluate the theoretical guarantees of our watermark approach on a set of real-world datasets. 
%
\paragraph{Datasets and Generators}
We evaluate our proposed watermarking technique and the baseline approaches on four real-world datasets of various sizes and distributions: Boston Housing and California Housing Price for regression task, as well as Adult and Wilt~\citep{misc_wilt_285} for classification task. For each dataset, we generate corresponding synthetic datasets using Gaussian Copula~\citep{masarotto2012gaussian}. We use Random Forest as the downsstream machine learning algorithm for all datasets. 
%
% For each dataset, we generate corresponding synthetic datasets using neural network-based methods~\cite{park2018data} and statistical-based generative methods~\cite{li2020sync}. Each of these methods for synthetic data generation possesses distinctive capabilities and features. For this paper, we employ CTGAN~\citep{xu2019modeling}, Gaussian Copula~\citep{masarotto2012gaussian}, and TVAE~\citep{xu2019modeling} which represent GAN-based~\citep{goodfellow2014generative}, copula-based~\citep{patki2016synthetic}, and VAE-based generators~\citep{kingma2013auto} respectively to generate tabular data. 

\paragraph{Utility}
%%%%%
% \begin{table}[t]
% \begin{tabular}{|l|c|c|c|c|cc|cc|}
% \hline
% \multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{Dataset}}} & \multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Not\\ watermarked\end{tabular}}} & \multirow{2}{*}{\textbf{Watermarked}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Watermarked \\ \& truncated\end{tabular}}} & \multicolumn{2}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Watermarked w/\\ 20\% cols drop\end{tabular}}} & \multicolumn{2}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Watermarked w/\\ 40\% cols drop\end{tabular}}} \\ \cline{6-9} 
% \multicolumn{1}{|c|}{}                                  &                                  &                                                                                    &                                       &                                                                                               & \multicolumn{1}{c|}{\textbf{FI}}                           & \textbf{Random}                          & \multicolumn{1}{c|}{\textbf{FI}}                           & \textbf{Random}                          \\ \hline
% \multirow{3}{*}{California}                             & CTGAN                            & 0.373                                                                              & 0.371                                 & 0.368                                                                                         & \multicolumn{1}{c|}{0.301}                                 & 0.242                                    & \multicolumn{1}{c|}{0.203}                                 & 0.256                                    \\
%                                                         & Copula                           & 0.370                                                                              & 0.376                                 & 0.376                                                                                         & \multicolumn{1}{c|}{0.347}                                 & 0.332                                    & \multicolumn{1}{c|}{0.31}                                  & 0.30                                     \\
%                                                         & TVAE                             & 0.797                                                                              & 0.799                                 & 0.798                                                                                         & \multicolumn{1}{c|}{0.448}                                 & 0.407                                    & \multicolumn{1}{c|}{0.385}                                 & 0.365                                    \\ \hline
% \multirow{3}{*}{Wilt}                                   & CTGAN                            & 0.731                                                                              & 0.733                                 & 0.733                                                                                         & \multicolumn{1}{c|}{0.575}                                 & 0.574                                    & \multicolumn{1}{c|}{0.563}                                 & 0.563                                    \\
%                                                         & Copula                           & 0.99                                                                               & 0.996                                 & 0.996                                                                                         & \multicolumn{1}{c|}{0.995}                                 & 0.994                                    & \multicolumn{1}{c|}{0.993}                                 & 0.993                                    \\
%                                                         & TVAE                             & 0.989                                                                              & 0.989                                 & 0.989                                                                                         & \multicolumn{1}{c|}{0.965}                                 & 0.977                                    & \multicolumn{1}{c|}{0.972}                                 & 0.803                                    \\ \hline
% \end{tabular}
% \caption{Accuracy of the downstream models under various attacks to the watermarked datasets. In particular, we provide accuracy for the original dataset and its watermarked counterpart. Additionally, we consider truncation as well as the column dropping separately that are typical preprocessing steps in a machine learning pipeline. We note that the effect of our watermarking technique is negligible in terms of accuracy in all cases while maintaining high detectability.}
% \label{table:utility}
% \end{table}

\begin{table*}[ht]
\centering
\begin{tabular}{|l|c|c|cccccc|}
\hline
\multicolumn{1}{|c|}{\multirow{3}{*}{\textbf{Dataset}}} &
  \multirow{3}{*}{\textbf{Method}} &
  \multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Not WM\end{tabular}}} &
  \multicolumn{6}{c|}{\textbf{Watermarked (WM)}} \\ \cline{4-9} 
\multicolumn{1}{|c|}{} &
   &
   &
  \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{WM}}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}WM and\\ Truncated\end{tabular}}}} &
  \multicolumn{2}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}WM and \\ 20\% cols drop\end{tabular}}} &
  \multicolumn{2}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}WM and \\ 40\% cols drop\end{tabular}}} \\ \cline{6-9} 
\multicolumn{1}{|c|}{} &
   &
   &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{\textbf{FI}} &
  \multicolumn{1}{c|}{\textbf{Random}} &
  \multicolumn{1}{c|}{\textbf{FI}} &
  \textbf{Random} \\ \hline
\multirow{3}{*}{California} &
  CTGAN &
  0.373 &
  \multicolumn{1}{c|}{0.371} &
  \multicolumn{1}{c|}{0.368} &
  \multicolumn{1}{c|}{0.301} &
  \multicolumn{1}{c|}{0.242} &
  \multicolumn{1}{c|}{0.203} &
  0.256 \\
 &
  Copula &
  0.370 &
  \multicolumn{1}{c|}{0.376} &
  \multicolumn{1}{c|}{0.376} &
  \multicolumn{1}{c|}{0.347} &
  \multicolumn{1}{c|}{0.332} &
  \multicolumn{1}{c|}{0.31} &
  0.30 \\
 &
  TVAE &
  0.797 &
  \multicolumn{1}{c|}{0.799} &
  \multicolumn{1}{c|}{0.798} &
  \multicolumn{1}{c|}{0.448} &
  \multicolumn{1}{c|}{0.407} &
  \multicolumn{1}{c|}{0.385} &
  0.365 \\ \hline
\multirow{3}{*}{Wilt} &
  CTGAN &
  0.731 &
  \multicolumn{1}{c|}{0.733} &
  \multicolumn{1}{c|}{0.733} &
  \multicolumn{1}{c|}{0.575} &
  \multicolumn{1}{c|}{0.574} &
  \multicolumn{1}{c|}{0.563} &
  0.563 \\
 &
  Copula &
  0.99 &
  \multicolumn{1}{c|}{0.996} &
  \multicolumn{1}{c|}{0.996} &
  \multicolumn{1}{c|}{0.995} &
  \multicolumn{1}{c|}{0.994} &
  \multicolumn{1}{c|}{0.993} &
  0.993 \\
 &
  TVAE &
  0.989 &
  \multicolumn{1}{c|}{0.989} &
  \multicolumn{1}{c|}{0.989} &
  \multicolumn{1}{c|}{0.965} &
  \multicolumn{1}{c|}{0.977} &
  \multicolumn{1}{c|}{0.972} &
  0.803 \\ \hline
\end{tabular}
\caption{Accuracy of the downstream models under various attacks to the watermarked datasets. In particular, we provide accuracy for the original dataset and its watermarked counterpart. Additionally, we consider truncation and the column dropping separately that are typical preprocessing steps in a machine learning pipeline. The effect of our watermarking technique is negligible in terms of accuracy in all cases while maintaining high detectability.}
\label{table:utility}
\end{table*}
%%%%%
% \begin{table*}[t]
% \centering
% \begin{tabular}{|l|l|c|c|c|cc|cc|}
% \hline
% \multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{Dataset}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Method}}} & \multirow{2}{*}{\textbf{No wm}} & \multirow{2}{*}{\textbf{Wm}} & \multirow{2}{*}{\textbf{wm+trunc 2 places}} & \multicolumn{2}{c|}{\textbf{wm with cols drop}}    & \multicolumn{2}{c|}{\textbf{Random pair wm with cols drop}} \\ \cline{6-9} 
% \multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{}                                 &                                 &                              &                                             & \multicolumn{1}{c|}{\textbf{20\%}} & \textbf{40\%} & \multicolumn{1}{c|}{\textbf{20\%}}      & \textbf{40\%}     \\ \hline

% California                                              & CTGAN                                                 & 0.373                              & 0.371                           & 0.368                                         & \multicolumn{1}{c|}{0.301}            & 0.203            & \multicolumn{1}{c|}{0.242}                 &        0.256           \\
%                                                         & Copula                                                & 0.370  & 0.376  & 0.376                                          & \multicolumn{1}{c|}{0.347}            & 0.31            & \multicolumn{1}{c|}{0.332}                 & 0.30                  \\
%                                                         & TVAE                                                  & 0.797  & 0.799  & 0.798                                          & \multicolumn{1}{c|}{0.4476}            & 0.385          & \multicolumn{1}{c|}{0.407}                 &      0.365             \\ \hline
% Wilt                                                    & CTGAN                                                 & 0.731                        & 0.733                      & 0.733                                     & \multicolumn{1}{c|}{0.575}          & 0.563         & \multicolumn{1}{c|}{0.574}                 &     0.563              \\
%                                                         & Copula                                                & 0.99                          & 0.996                      & 0.996                                     & \multicolumn{1}{c|}{0.995}            & 0.993           & \multicolumn{1}{c|}{0.994}                 &      0.993             \\
%                                                         & TVAE                                                  & 0.989                         & 0.989                      & 0.989                                    & \multicolumn{1}{c|}{0.965}            & 0.972            & \multicolumn{1}{c|}{0.977}                 &   0.803                \\ \hline
% \end{tabular}
% \caption{Accuracy of the downstream models under various attacks to the watermarked datasets. In particular, we provide accuracy for the original dataset and its watermarked counterpart. Additionally, we consider truncation as well as the column dropping separately that are typical preprocessing steps in a machine learning pipeline. We note that the affect of our watermarking techniques is negligible in terms of accuracy in all cases while maintaining high detectability. \dscomment{do we feel like we've provided evidence to claim high detectability?}\vpcomment{If you finish that experiment with number of pairs, we can make that point.}}
% \end{table*}
%%%%

For evaluating utility, we focus on machine learning (ML) efficiency ~\citep{xu2019modeling}. In more detail, ML efficiency quantifies the performance of classification or regression models that are trained on synthetic data and evaluated on the real test set. In our experiment, we evaluate ML efficiency with respect to the Random Forest classifier, which are then evaluated on real testing sets. Classification performances are evaluated by the accuracy score. To explore the performance of our tabular watermark on real-world data, we sample from each generative model a generated dataset with the size of a real training set. For each setup, we create 5 watermarked training sets to measure the accuracy score. For reproducibility, we set a specific random seed to ensure that the data deformation and model training effects are repeatable on a similar hardware and software stack. To eliminate the randomness of the results, the experimental outcomes are averaged over multiple runs from each watermarked training set.

We watermark each of the generated datasets using a \textit{bin size} of $10^{-2}$ and thus only consider columns that contain floating point numbers with at least 2 decimal places. This choice follows from the practical consideration that watermarking with this bin size involves perturbing up to 2 decimal places, and watermarking any original columns that did not already contain values with this property may make it obvious to an outside party upon receiving the dataset that this specific section of the data has been manipulated.

We also consider two common data science preprocessing steps that downstream users of the watermarked datasets might conduct: truncation and dropping the least important columns. We aim to determine if the application of our watermark in conjunction with these operations  For the former, we truncate to 2 decimal places. For the latter, we investigate dropping the lowest 20\% and 40\% of columns in each case, considering when the data is watermarked both with and without the feature importance-based pairing scheme. 

We find that the effect of our watermarking technique is negligible in terms of accuracy in all cases while maintaining high detectability as seen in Table \ref{table:utility}.

\subsection{Spoofing}
\label{sec:spoofing}
\begin{figure*}[t]
    \centering
    \begin{subfigure}[b]{0.49\linewidth}
        \includegraphics[height=5cm]{figures/inhouse_spoof_exp.png}
    \caption{Spoofing: our watermark}
    \label{fig:spoofing-pairs}
    \end{subfigure}
    %
    \hfill
    %
    \begin{subfigure}[b]{0.49\linewidth}
    \centering
        \includegraphics[height=4.5cm]{figures/guang_spoof.png}
    \caption{Spoofing: \citet{he2024watermarkinggenerativetabulardata}'s watermark}
    \label{fig:spoofing-guang}
    \end{subfigure}
    \caption{
    (a) $p$-value calculated with our watermark approach under spoofing attack (\Cref{alg:fractional}). Our approach is highly robust as the spoofing algorithm as well as the percent of data processed has no effect on our dataset. (b) $p$-value calculated with WGTD watermark~\citep{he2024watermarkinggenerativetabulardata}. As the percentage of data processed increases, the $p$-value decreases. As the percent of data processed increases near $40 \%$, the $p$-value of \citet{he2024watermarkinggenerativetabulardata}'s watermark is already below $0.05$ and the watermark can be spoofed using \Cref{alg:fractional}.} 
    \label{fig:spoof-data}
\end{figure*}

We introduce a novel method (\Cref{alg:fractional}) to validate the robustness of our algorithm and the WGTD watermark~\citep{he2024watermarkinggenerativetabulardata} against spoofing attack. This spoofing algorithm is designed to subtly alter a dataset by modifying the decimal points of its element so that the dataset appears to be watermarked. The process begins by computing the integers and fractional parts of a synthetic dataset and a reference watermarked dataset. For the experiment shown below (\Cref{fig:spoofing-guang}), we generated a synthetic dataset of the original unwatermarked dataset to act as our target. For each element in the synthetic dataset, the algorithm identifies the closest fractional part from the watermarked dataset to the current element. If the element is non-negative, the fractional part is added to the integer part. This method ensures that the watermark is embedded in a way that is minimally invasive, preserving the fidelity, detectability, overall structure and integrity of the original data while introducing a subtle, detectable pattern. The experimental results are in \Cref{fig:spoof-data}. 

Using \Cref{alg:fractional} (detailed in \Cref{appendix:spoofing}), we can successfully spoof the WGTD watermark scheme~\citep{he2024watermarkinggenerativetabulardata} after replacing about $40\%$ of the synthetic dataset. That is, the spoofed dataset generated from \Cref{alg:fractional} will be classified as `watermarked' by the~\citet{he2024watermarkinggenerativetabulardata}'s detector as the $p$-value drops below $0.05$. On the other hand, our watermark approach (\Cref{alg:tabular}) cannot be spoofed by using \Cref{alg:fractional} at all. Even after all data points in the synthetic dataset have been processed, the $p$-value from our detection hypothesis test (\Cref{sec:dectection}) still remains above $0.05$. This result shows that our watermark approach is more robust to simple spoofing attack compared to prior work of \citet{he2024watermarkinggenerativetabulardata} by leveraging the structure of the tabular dataset. 
%
%


==> prelim.tex <==
\section{Problem Formulation}
\label{sec:prelim}
%
\paragraph{Notation.} For $n \in \mathbb{N}^{+}$, we write $[n]$ to denote $\{1,\cdots,n \}$. For a matrix $\bX \in \mathbb{R}^{m \times 2n}$, we denote the entry-wise $\ell_\infty$-norm of $\bX$ as $\norm{\bX}_\infty = \max_{i \in [m], j \in [2n]} \abs{\bX_{i,j}}$. For an interval $g = [a, b]$, we denote the center of $g$ as $\mathrm{center}(g) = \nicefrac{(a + b)}{2}$. Given a real number $x$, $\lfloor x \rfloor$ is the largest integer that is less than or equal to $x$, and $x^\circ = x - \lfloor x \rfloor$ denotes its fractional part.

We consider an original tabular dataset $\bX \in [0,1]^{m \times 2n}$ with each column containing $m$ i.i.d data points from a (possibly unknown) distribution $F_i$ for $i \in [2n]$.
Our objective is to generate a watermarked version of this data, denoted $\bX_w$, with the following properties:
%
\begin{enumerate}[label=(\roman*)]
    \item \textbf{Fidelity}: the watermarked dataset $\bX_w$ is close to the original data set $\bX$ to maintain high fidelity, measured through $L_\infty$ and Wasserstein distances; \label{prop:fidelity}
    %
    \item \textbf{Detectability}: the watermarked dataset $\bX_w$ can be reliably identified through the one-proportion $z$-test using only few row samples;
    %
    \item \textbf{Robustness}: the watermarked dataset $\bX_w$ is robust against multiple methods of oblivious `attack' commonly observed in data science; 
    %
    \item \textbf{Security}: it is difficult for an adversary to learn the underlying watermarking scheme without considerable computational efforts.  
\end{enumerate}
%
In our analysis, we only focus on embedding the watermark in the continuous features of a tabular dataset. While a real-world tabular dataset may contain many categorical features, embedding the watermark in these features through a small perturbation of its value may cause significant changes in the meaning for the entire row. Given a dataset $\bX$ with mixed data types, one may run our algorithm on a smaller dataset $\bX' \subseteq \bX$ with same number of rows and only continuous features. After the watermark has been embedded in $\bX'$ to get $\bX'_w$, a watermarked version of the original dataset $\bX$ can be reconstructed by replacing the continuous features of $\bX$ with its watermarked versions from $\bX'_w$. We leave the study of watermarking categorical features in tabular datasets for future work.



==> truncation.tex <==
\subsection{Robustness to Truncation}
\label{sec:truncation}
%
\AS{This section goes away in the final version. We need to integrate it with the previous section on robustness. I have just written down one sentence at the moment but we can write more.}
%
In addition to feature selection, one can also `attack' the watermarked dataset by directly modifying elements in the dataset. In particular, we are interested in \emph{truncation} attack, where the one systematically reduces the number of digits after the decimal point of all elements in the dataset. Formally, let $\trunc: \mathbb{R} \rightarrow \mathbb{R}$ be the truncation function defined as:
\begin{equation}
    \xtr = \trunc(x,p) = \frac{\floor{10^p \cdot x}}{10^p}
    %
    \label{eq:trunc}
\end{equation}
%
That is, for all $x \in \bX_w$, the adversary truncates the digits in the mantissa of $x$ to $\xtr \in \mathbb{R}$ with $p$ digits in the mantissa. For example, with $x = 0.369$ and $p=2$, the modified cell $\xtr$ becomes $0.36$. In the following analysis, we focus on the case where $p = 2$, \ie all values are truncated to $2$ decimal places. Extension to more digits in the mantissa follows the same analysis. 

First, we determine how this truncation operation influence the distribution of watermarked elements in green intervals. When a watermarked element $x$ in a $value$ column is truncated to $\xtr$, it can fall out of the original green interval if the bins $[0, \nicefrac{1}{b}], \cdots, [\nicefrac{b-1}{b}, 1]$ and the hundredth grid points $\{0, 0.01, 0.02, \cdots, 0.99 ,1\}$ are not perfectly aligned.
To illustrate this phenomenon, we presented a stylized example where \Cref{alg:tabular} uses $b = 150$ bins in its watermarking procedure. Then, in the second bin $I_2 = [\nicefrac{1}{150}, \nicefrac{2}{150}]$, all $x \in [\nicefrac{1}{150}, 0.01)$ will be truncated to $\xtr = 0.0 \in I_1$. If $I_1$ is a red interval then the truncation operation has successfully moved elements out of the green intervals. In the following theorem, we show the probability of successful truncation attack as a function of the bin width. 
%
\begin{theorem}
    Let $p$ be the precision of a given a watermarked element $x \in I_j = [\nicefrac{j-1}{b}, \nicefrac{j}{b}]$ and the truncation function defined in~\Cref{eq:trunc}. Then, the probability that the truncated element $\xtr$ falls out of its original green interval is 
    %
    \begin{equation*}
        \Pr [\xtr \notin I_j] = \frac{(b-1)^{10^p} + b^{10^p-1}(c \cdot b - j + 1)}{b^{10^p}} 
    \end{equation*}
    %
    where $c \in \{0, 0.01, \cdots, 0.99 \}$ are the left grid points of $I_j$ intervals. 
\label{thm:truncation}
\end{theorem}
%
Intuitively, with larger bin size $\nicefrac{1}{b}$, the probability that our proposed watermarking scheme can withstand truncation attack increases as the truncated elements are more likely to fall into the same bins as the original elements. On the other hand, when the bins are more fine-grained, truncation would almost surely move the watermarked data outside of the original intervals. This result presents an interesting trade-off between smaller bin width for higher fidelity (see \Cref{thm:fidelity}) and bigger bin width for better robustness, which has not been studied in prior work on watermarking tabular data. 
With this insight, we can choose the bin width to be the same as the truncation grid size, \ie $\nicefrac{1}{b} = \nicefrac{1}{10^p}$ or $b = 10^p$ to ensure high fidelity and robustness.

